How Robust are LLMs to In-Context Majority Label Bias?

In the In-Context Learning (ICL) setup, various forms of label biases can manifest. One such manifestation is majority label bias, which arises when the distribution of labeled examples in the in-context samples is skewed towards one or more specific classes making Large Language Models (LLMs) more prone to predict those labels. Such discrepancies can arise from various factors, including logistical constraints, inherent biases in data collection methods, limited access to diverse data sources, etc. which are unavoidable in a real-world industry setup. In this work, we study the robustness of in-context learning in LLMs to shifts that occur due to majority label bias within the purview of text classification tasks. Prior works have shown that in-context learning with LLMs is susceptible to such biases. In our study, we go one level deeper and show that the robustness boundary varies widely for different models and tasks, with certain LLMs being highly robust (~90%) to majority label bias. Additionally, our findings also highlight the impact of model size and the richness of instructional prompts contributing towards model robustness. We restrict our study to only publicly available open-source models to ensure transparency and reproducibility.

==> rof1.tex <==
\begin{table*}[ht]
% \begin{tabular}{ccccccccccc}
\tiny
\centering
\begin{tabular}
% {|p{1.25cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}|p{0.95cm}}
{|p{0.75cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}}
% Dataset       & OL-7B-wo-instruction & OL-7B-w-instruction & OL-13B-wo-instruction & OL-13B-w-instruction & Falcon-40B-wo-instruction & Falcon-40B-w-instruction & MPT-7B-wo-instruction & MPT-7B-w-instruction & MPT-30B-wo-instruction & MPT-30B-w-instruction & BERT  & Random Classifier \\ 
\hline
 & OL-7B-wo & OL-7B-w & OL-13B-wo & OL-13B-w & Falcon-40B-wo & Falcon-40B-w &  MPT-7B-wo & MPT-7B-w& MPT-30B-wo & MPT-30B-w \\ \hline
\multicolumn{11}{|c|}{\textbf{BoolQ}}     \\  \hline
\textit{RB@10 }         & 0.546                & 0.636               & 0.546                 & 0.727                & 0.546                     & \textbf{0.909}                    & 0.455                 & 0.818                & 0.636                  & 0.818                            \\
wt-F1       & 0.450                & 0.443               & 0.469                 & 0.490                & 0.593                     & \textbf{0.605}                    & 0.436                 & 0.548                & 0.545                  & 0.598                               \\
std dev & 0.144                & 0.141               & 0.124                 & 0.107                & 0.112                     & 0.055          &   0.143       & 0.053                 & 0.127                & \textbf{0.049}                                                 \\ \hline
\multicolumn{11}{|c|}{\textbf{RTE}}     \\  \hline
\textit{RB@10 }         & 0.727                & 0.818               & 0.818                 & 0.909                & 0.727                     & \textbf{1.000}                    & 0.546                 & 0.636                & 0.909                  & \textbf{1.000}                             \\
wt-F1       & 0.490                & 0.565               & 0.659                 & 0.618                & 0.706                     & 0.744                    & 0.570                 & 0.601                & 0.756                  & \textbf{0.781}                           \\
std dev & 0.076                & 0.040               & 0.084                 & 0.064                & 0.083                     & 0.031                    & 0.142                 & 0.064                & 0.083                  & \textbf{0.022}                                \\ \hline
\multicolumn{11}{|c|}{\textbf{Covid-5G}}     \\  \hline
\textit{RB@10}          & 0.400                & 0.467               & 0.200                 & 0.267                & 0.333                     & \textbf{0.533}                    & 0.000                 & 0.400                & 0.200                  & 0.467                          \\
wt-F1       & 0.299                & 0.284               & 0.319                 & 0.454                & 0.484                     & \textbf{0.645}                    & 0.341                 & 0.397                & 0.455                  & 0.581                             \\
std dev& 0.123                & 0.066               & 0.123                 & 0.132                & 0.169                     & \textbf{0.079}                    & 0.121                 & 0.106                & 0.183                  & 0.113                               \\ \hline
\end{tabular}
\caption{\small Comparison of RB@10, Average and Std. deviation of weighted F1 across various LLMs for the three datasets. The best results are highlighted in \textbf{bold}. Higher the RB@10, the more robust the peak performance.}
\label{tab:rb_f1}
\end{table*}
